Enhancing Routing in SD-EONs through Reinforcement Learning: A Comparative Analysis

This paper presents an optimization framework for routing in software-defined elastic optical networks using reinforcement learning algorithms. We specifically implement and compare the epsilon-greedy bandit, upper confidence bound (UCB) bandit, and Q-learning algorithms to traditional methods such as K-Shortest Paths with First-Fit core and spectrum assignment (KSP-FF) and Shortest Path with First-Fit (SPF-FF) algorithms. Our results show that Q-learning significantly outperforms traditional methods, achieving a reduction in blocking probability (BP) of up to 58.8% over KSP-FF, and 81.9% over SPF-FF under lower traffic volumes. For higher traffic volumes, Q-learning maintains superior performance with BP reductions of 41.9% over KSP-FF and 70.1% over SPF-FF. These findings demonstrate the efficacy of reinforcement learning in enhancing network performance and resource utilization in dynamic and complex environments.

==> plots/erlang_1000/NSFNet/k4.tex <==
% k4.tex

\begin{tikzpicture}
\begin{axis}[
    title={NSFNet Blocking Probability vs. Episodes},
    xlabel={Episodes},
    ylabel={Blocking Probability},
    grid,
    scaled y ticks=false,
    yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/fixed zerofill,
        /pgf/number format/precision=3,
    },
    xmax=100,
    xmin=-1,
    width=0.83\linewidth,
    height=0.73\linewidth,
    legend style={
        at={(0.99,0.68)},
        anchor=north east,
        legend cell align=left,
        font=\scriptsize,
    },
]

\addplot[
    no markers,
    solid,
    color=blue,
    line width=0.9pt,
] table [x=episodes, y=q_learning, col sep=comma] {data/erlang_1000/k4/NSFNet/best_performing.csv};
\addlegendentry{Q-Learning}

\addplot[
    no markers,
    solid,
    color=red,
    line width=0.9pt,
] table [x=episodes, y=epsilon_greedy_bandit, col sep=comma] {data/erlang_1000/k4/NSFNet/best_performing.csv};
\addlegendentry{Epsilon-Greedy Bandit}

\addplot[
    no markers,
    solid,
    color=gray,
    line width=0.9pt,
] table [x=episodes, y=ucb_bandit, col sep=comma] {data/erlang_1000/k4/NSFNet/best_performing.csv};
\addlegendentry{UCB Bandit}

\addplot[
    no markers,
    dashed,
    color=green,
    line width=0.9pt,
] table [x=episodes, y=spf, col sep=comma] {data/erlang_1000/k4/NSFNet/best_performing.csv};
\addlegendentry{SPF-FF}

\addplot[
    no markers,
    dashed,
    color=orange,
    line width=0.9pt,
] table [x=episodes, y=ksp, col sep=comma] {data/erlang_1000/k4/NSFNet/best_performing.csv};
\addlegendentry{KSP-FF $k=4$}

\end{axis}
\end{tikzpicture}

==> plots/erlang_1000/NSFNet/k5.tex <==
% k5.tex

\begin{tikzpicture}
\begin{axis}[
    title={NSFNet Blocking Probability vs. Episodes},
    xlabel={Episodes},
    ylabel={Blocking Probability},
    grid,
    scaled y ticks=false,
    yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/fixed zerofill,
        /pgf/number format/precision=3,
    },
    xmax=100,
    xmin=-1,
    width=0.83\linewidth,
    height=0.73\linewidth,
    legend style={
        at={(0.99,0.99)},
        anchor=north east,
        legend cell align=left,
        font=\scriptsize,
    },
]

\addplot[
    no markers,
    solid,
    color=blue,
    line width=0.9pt,
] table [x=episodes, y=q_learning, col sep=comma] {data/erlang_1000/k5/NSFNet/best_performing.csv};
\addlegendentry{Q-Learning}

\addplot[
    no markers,
    solid,
    color=red,
    line width=0.9pt,
] table [x=episodes, y=epsilon_greedy_bandit, col sep=comma] {data/erlang_1000/k5/NSFNet/best_performing.csv};
\addlegendentry{Epsilon-Greedy Bandit}

\addplot[
    no markers,
    solid,
    color=gray,
    line width=0.9pt,
] table [x=episodes, y=ucb_bandit, col sep=comma] {data/erlang_1000/k5/NSFNet/best_performing.csv};
\addlegendentry{UCB Bandit}

\addplot[
    no markers,
    dashed,
    color=green,
    line width=0.9pt,
] table [x=episodes, y=spf, col sep=comma] {data/erlang_1000/k5/NSFNet/best_performing.csv};
\addlegendentry{SPF-FF}

\addplot[
    no markers,
    dashed,
    color=orange,
    line width=0.9pt,
] table [x=episodes, y=ksp, col sep=comma] {data/erlang_1000/k5/NSFNet/best_performing.csv};
\addlegendentry{KSP-FF $k=5$}

\end{axis}
\end{tikzpicture}

==> plots/erlang_1000/Pan-European/k3.tex <==
% k3.tex

\begin{tikzpicture}
\begin{axis}[
    title={Pan-European Blocking Probability vs. Episodes},
    xlabel={Episodes},
    ylabel={Blocking Probability},
    grid,
    scaled y ticks=false,
    yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/fixed zerofill,
        /pgf/number format/precision=3,
    },
    xmax=100,
    xmin=-1,
    width=0.83\linewidth,
    height=0.73\linewidth,
    legend style={
        at={(0.99,0.8)},
        anchor=north east,
        legend cell align=left,
        font=\scriptsize,
    },
]

\addplot[
    no markers,
    solid,
    color=blue,
    line width=0.9pt,
] table [x=episodes, y=q_learning, col sep=comma] {data/erlang_1000/k3/Pan-European/best_performing.csv};
\addlegendentry{Q-Learning}

\addplot[
    no markers,
    solid,
    color=red,
    line width=0.9pt,
] table [x=episodes, y=epsilon_greedy_bandit, col sep=comma] {data/erlang_1000/k3/Pan-European/best_performing.csv};
\addlegendentry{Epsilon-Greedy Bandit}

\addplot[
    no markers,
    solid,
    color=gray,
    line width=0.9pt,
] table [x=episodes, y=ucb_bandit, col sep=comma] {data/erlang_1000/k3/Pan-European/best_performing.csv};
\addlegendentry{UCB Bandit}

\addplot[
    no markers,
    dashed,
    color=green,
    line width=0.9pt,
] table [x=episodes, y=spf, col sep=comma] {data/erlang_1000/k3/Pan-European/best_performing.csv};
\addlegendentry{SPF-FF}

\addplot[
    no markers,
    dashed,
    color=orange,
    line width=0.9pt,
] table [x=episodes, y=ksp, col sep=comma] {data/erlang_1000/k3/Pan-European/best_performing.csv};
\addlegendentry{KSP-FF $k=3$}

\end{axis}
\end{tikzpicture}

==> plots/erlang_1000/Pan-European/k4.tex <==
% k4.tex

\begin{tikzpicture}
\begin{axis}[
    title={Pan-European Blocking Probability vs. Episodes},
    xlabel={Episodes},
    ylabel={Blocking Probability},
    grid,
    scaled y ticks=false,
    yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/fixed zerofill,
        /pgf/number format/precision=3,
    },
    xmax=100,
    xmin=-1,
    width=0.83\linewidth,
    height=0.73\linewidth,
    legend style={
        at={(0.99,0.8)},
        anchor=north east,
        legend cell align=left,
        font=\scriptsize,
    },
]

\addplot[
    no markers,
    solid,
    color=blue,
    line width=0.9pt,
] table [x=episodes, y=q_learning, col sep=comma] {data/erlang_1000/k4/Pan-European/best_performing.csv};
\addlegendentry{Q-Learning}

\addplot[
    no markers,
    solid,
    color=red,
    line width=0.9pt,
] table [x=episodes, y=epsilon_greedy_bandit, col sep=comma] {data/erlang_1000/k4/Pan-European/best_performing.csv};
\addlegendentry{Epsilon-Greedy Bandit}

\addplot[
    no markers,
    solid,
    color=gray,
    line width=0.9pt,
] table [x=episodes, y=ucb_bandit, col sep=comma] {data/erlang_1000/k4/Pan-European/best_performing.csv};
\addlegendentry{UCB Bandit}

\addplot[
    no markers,
    dashed,
    color=green,
    line width=0.9pt,
] table [x=episodes, y=spf, col sep=comma] {data/erlang_1000/k4/Pan-European/best_performing.csv};
\addlegendentry{SPF-FF}

\addplot[
    no markers,
    dashed,
    color=orange,
    line width=0.9pt,
] table [x=episodes, y=ksp, col sep=comma] {data/erlang_1000/k4/Pan-European/best_performing.csv};
\addlegendentry{KSP-FF $k=4$}

\end{axis}
\end{tikzpicture}

==> plots/erlang_1000/Pan-European/k5.tex <==
% k5.tex

\begin{tikzpicture}
\begin{axis}[
    title={Pan-European Blocking Probability vs. Episodes},
    xlabel={Episodes},
    ylabel={Blocking Probability},
    grid,
    scaled y ticks=false,
    yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/fixed zerofill,
        /pgf/number format/precision=3,
    },
    xmax=100,
    xmin=-1,
    width=0.83\linewidth,
    height=0.73\linewidth,
    legend style={
        at={(0.99,0.8)},
        anchor=north east,
        legend cell align=left,
        font=\scriptsize,
    },
]

\addplot[
    no markers,
    solid,
    color=blue,
    line width=0.9pt,
] table [x=episodes, y=q_learning, col sep=comma] {data/erlang_1000/k5/Pan-European/best_performing.csv};
\addlegendentry{Q-Learning}

\addplot[
    no markers,
    solid,
    color=red,
    line width=0.9pt,
] table [x=episodes, y=epsilon_greedy_bandit, col sep=comma] {data/erlang_1000/k5/Pan-European/best_performing.csv};
\addlegendentry{Epsilon-Greedy Bandit}

\addplot[
    no markers,
    solid,
    color=gray,
    line width=0.9pt,
] table [x=episodes, y=ucb_bandit, col sep=comma] {data/erlang_1000/k5/Pan-European/best_performing.csv};
\addlegendentry{UCB Bandit}

\addplot[
    no markers,
    dashed,
    color=green,
    line width=0.9pt,
] table [x=episodes, y=spf, col sep=comma] {data/erlang_1000/k5/Pan-European/best_performing.csv};
\addlegendentry{SPF-FF}

\addplot[
    no markers,
    dashed,
    color=orange,
    line width=0.9pt,
] table [x=episodes, y=ksp, col sep=comma] {data/erlang_1000/k5/Pan-European/best_performing.csv};
\addlegendentry{KSP-FF $k=5$}

\end{axis}
\end{tikzpicture}

==> plots/erlang_1000/USNet/k3.tex <==
% k3.tex

\begin{tikzpicture}
\begin{axis}[
    title={USNet Blocking Probability vs. Episodes},
    xlabel={Episodes},
    ylabel={Blocking Probability},
    grid,
    scaled y ticks=false,
    yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/fixed zerofill,
        /pgf/number format/precision=3,
    },
    xmax=100,
    xmin=-1,
    width=0.83\linewidth,
    height=0.73\linewidth,
    legend style={
        at={(0.99,0.8)},
        anchor=north east,
        legend cell align=left,
        font=\scriptsize,
    },
]

\addplot[
    no markers,
    solid,
    color=blue,
    line width=0.9pt,
] table [x=episodes, y=q_learning, col sep=comma] {data/erlang_1000/k3/USNet/best_performing.csv};
\addlegendentry{Q-Learning}

\addplot[
    no markers,
    solid,
    color=red,
    line width=0.9pt,
] table [x=episodes, y=epsilon_greedy_bandit, col sep=comma] {data/erlang_1000/k3/USNet/best_performing.csv};
\addlegendentry{Epsilon-Greedy Bandit}

\addplot[
    no markers,
    solid,
    color=gray,
    line width=0.9pt,
] table [x=episodes, y=ucb_bandit, col sep=comma] {data/erlang_1000/k3/USNet/best_performing.csv};
\addlegendentry{UCB Bandit}

\addplot[
    no markers,
    dashed,
    color=green,
    line width=0.9pt,
] table [x=episodes, y=spf, col sep=comma] {data/erlang_1000/k3/USNet/best_performing.csv};
\addlegendentry{SPF-FF}

\addplot[
    no markers,
    dashed,
    color=orange,
    line width=0.9pt,
] table [x=episodes, y=ksp, col sep=comma] {data/erlang_1000/k3/USNet/best_performing.csv};
\addlegendentry{KSP-FF $k=3$}

\end{axis}
\end{tikzpicture}

==> plots/erlang_1000/USNet/k4.tex <==
% k4.tex

\begin{tikzpicture}
\begin{axis}[
    title={USNet Blocking Probability vs. Episodes},
    xlabel={Episodes},
    ylabel={Blocking Probability},
    grid,
    scaled y ticks=false,
    yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/fixed zerofill,
        /pgf/number format/precision=3,
    },
    xmax=100,
    xmin=-1,
    width=0.83\linewidth,
    height=0.73\linewidth,
    legend style={
        at={(0.99,0.8)},
        anchor=north east,
        legend cell align=left,
        font=\scriptsize,
    },
]

\addplot[
    no markers,
    solid,
    color=blue,
    line width=0.9pt,
] table [x=episodes, y=q_learning, col sep=comma] {data/erlang_1000/k4/USNet/best_performing.csv};
\addlegendentry{Q-Learning}

\addplot[
    no markers,
    solid,
    color=red,
    line width=0.9pt,
] table [x=episodes, y=epsilon_greedy_bandit, col sep=comma] {data/erlang_1000/k4/USNet/best_performing.csv};
\addlegendentry{Epsilon-Greedy Bandit}

\addplot[
    no markers,
    solid,
    color=gray,
    line width=0.9pt,
] table [x=episodes, y=ucb_bandit, col sep=comma] {data/erlang_1000/k4/USNet/best_performing.csv};
\addlegendentry{UCB Bandit}

\addplot[
    no markers,
    dashed,
    color=green,
    line width=0.9pt,
] table [x=episodes, y=spf, col sep=comma] {data/erlang_1000/k4/USNet/best_performing.csv};
\addlegendentry{SPF-FF}

\addplot[
    no markers,
    dashed,
    color=orange,
    line width=0.9pt,
] table [x=episodes, y=ksp, col sep=comma] {data/erlang_1000/k4/USNet/best_performing.csv};
\addlegendentry{KSP-FF $k=4$}

\end{axis}
\end{tikzpicture}

==> plots/erlang_1000/USNet/k5.tex <==
% k5.tex

\begin{tikzpicture}
\begin{axis}[
    title={USNet Blocking Probability vs. Episodes},
    xlabel={Episodes},
    ylabel={Blocking Probability},
    grid,
    scaled y ticks=false,
    yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/fixed zerofill,
        /pgf/number format/precision=3,
    },
    xmax=100,
    xmin=-1,
    width=0.83\linewidth,
    height=0.73\linewidth,
    legend style={
        at={(0.99,0.8)},
        anchor=north east,
        legend cell align=left,
        font=\scriptsize,
    },
]

\addplot[
    no markers,
    solid,
    color=blue,
    line width=0.9pt,
] table [x=episodes, y=q_learning, col sep=comma] {data/erlang_750/k5/USNet/best_performing.csv};
\addlegendentry{Q-Learning}

\addplot[
    no markers,
    solid,
    color=red,
    line width=0.9pt,
] table [x=episodes, y=epsilon_greedy_bandit, col sep=comma] {data/erlang_1000/k5/USNet/best_performing.csv};
\addlegendentry{Epsilon-Greedy Bandit}

\addplot[
    no markers,
    solid,
    color=gray,
    line width=0.9pt,
] table [x=episodes, y=ucb_bandit, col sep=comma] {data/erlang_1000/k5/USNet/best_performing.csv};
\addlegendentry{UCB Bandit}

\addplot[
    no markers,
    dashed,
    color=green,
    line width=0.9pt,
] table [x=episodes, y=spf, col sep=comma] {data/erlang_1000/k5/USNet/best_performing.csv};
\addlegendentry{SPF-FF}

\addplot[
    no markers,
    dashed,
    color=orange,
    line width=0.9pt,
] table [x=episodes, y=ksp, col sep=comma] {data/erlang_1000/k5/USNet/best_performing.csv};
\addlegendentry{KSP-FF $k=5$}

\end{axis}
\end{tikzpicture}

==> plots/erlang_750/NSFNet/k4.tex <==
% k4.tex

\begin{tikzpicture}
\begin{axis}[
    title={NSFNet Blocking Probability vs. Episodes},
    xlabel={Episodes},
    ylabel={Blocking Probability},
    grid,
    scaled y ticks=false,
    yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/fixed zerofill,
        /pgf/number format/precision=3,
    },
    xmax=100,
    xmin=-1,
    width=0.83\linewidth,
    height=0.73\linewidth,
    legend style={
        at={(0.99,0.68)},
        anchor=north east,
        legend cell align=left,
        font=\scriptsize,
    },
]

\addplot[
    no markers,
    solid,
    color=blue,
    line width=0.9pt,
] table [x=episodes, y=q_learning, col sep=comma] {data/erlang_750/k4/NSFNet/best_performing.csv};
\addlegendentry{Q-Learning}

\addplot[
    no markers,
    solid,
    color=red,
    line width=0.9pt,
] table [x=episodes, y=epsilon_greedy_bandit, col sep=comma] {data/erlang_750/k4/NSFNet/best_performing.csv};
\addlegendentry{Epsilon-Greedy Bandit}

\addplot[
    no markers,
    solid,
    color=gray,
    line width=0.9pt,
] table [x=episodes, y=ucb_bandit, col sep=comma] {data/erlang_750/k4/NSFNet/best_performing.csv};
\addlegendentry{UCB Bandit}

\addplot[
    no markers,
    dashed,
    color=green,
    line width=0.9pt,
] table [x=episodes, y=spf, col sep=comma] {data/erlang_750/k4/NSFNet/best_performing.csv};
\addlegendentry{SPF-FF}

\addplot[
    no markers,
    dashed,
    color=orange,
    line width=0.9pt,
] table [x=episodes, y=ksp, col sep=comma] {data/erlang_750/k4/NSFNet/best_performing.csv};
\addlegendentry{KSP-FF $k=4$}

\end{axis}
\end{tikzpicture}

==> plots/erlang_750/NSFNet/k5.tex <==
% k5.tex

\begin{tikzpicture}
\begin{axis}[
    title={NSFNet Blocking Probability vs. Episodes},
    xlabel={Episodes},
    ylabel={Blocking Probability},
    grid,
    scaled y ticks=false,
    yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/fixed zerofill,
        /pgf/number format/precision=3,
    },
    xmax=100,
    xmin=-1,
    width=0.83\linewidth,
    height=0.73\linewidth,
    legend style={
        at={(0.99,0.99)},
        anchor=north east,
        legend cell align=left,
        font=\scriptsize,
    },
]

\addplot[
    no markers,
    solid,
    color=blue,
    line width=0.9pt,
] table [x=episodes, y=q_learning, col sep=comma] {data/erlang_750/k5/NSFNet/best_performing.csv};
\addlegendentry{Q-Learning}

\addplot[
    no markers,
    solid,
    color=red,
    line width=0.9pt,
] table [x=episodes, y=epsilon_greedy_bandit, col sep=comma] {data/erlang_750/k5/NSFNet/best_performing.csv};
\addlegendentry{Epsilon-Greedy Bandit}

\addplot[
    no markers,
    solid,
    color=gray,
    line width=0.9pt,
] table [x=episodes, y=ucb_bandit, col sep=comma] {data/erlang_750/k5/NSFNet/best_performing.csv};
\addlegendentry{UCB Bandit}

\addplot[
    no markers,
    dashed,
    color=green,
    line width=0.9pt,
] table [x=episodes, y=spf, col sep=comma] {data/erlang_750/k5/NSFNet/best_performing.csv};
\addlegendentry{SPF-FF}

\addplot[
    no markers,
    dashed,
    color=orange,
    line width=0.9pt,
] table [x=episodes, y=ksp, col sep=comma] {data/erlang_750/k5/NSFNet/best_performing.csv};
\addlegendentry{KSP-FF $k=5$}

\end{axis}
\end{tikzpicture}

==> plots/erlang_750/Pan-European/k3.tex <==
% k3.tex

\begin{tikzpicture}
\begin{axis}[
    title={Pan-European Blocking Probability vs. Episodes},
    xlabel={Episodes},
    ylabel={Blocking Probability},
    grid,
    scaled y ticks=false,
    yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/fixed zerofill,
        /pgf/number format/precision=3,
    },
    xmax=100,
    xmin=-1,
    width=0.83\linewidth,
    height=0.73\linewidth,
    legend style={
        at={(0.99,0.8)},
        anchor=north east,
        legend cell align=left,
        font=\scriptsize,
    },
]

\addplot[
    no markers,
    solid,
    color=blue,
    line width=0.9pt,
] table [x=episodes, y=q_learning, col sep=comma] {data/erlang_750/k3/Pan-European/best_performing.csv};
\addlegendentry{Q-Learning}

\addplot[
    no markers,
    solid,
    color=red,
    line width=0.9pt,
] table [x=episodes, y=epsilon_greedy_bandit, col sep=comma] {data/erlang_750/k3/Pan-European/best_performing.csv};
\addlegendentry{Epsilon-Greedy Bandit}

\addplot[
    no markers,
    solid,
    color=gray,
    line width=0.9pt,
] table [x=episodes, y=ucb_bandit, col sep=comma] {data/erlang_750/k3/Pan-European/best_performing.csv};
\addlegendentry{UCB Bandit}

\addplot[
    no markers,
    dashed,
    color=green,
    line width=0.9pt,
] table [x=episodes, y=spf, col sep=comma] {data/erlang_750/k3/Pan-European/best_performing.csv};
\addlegendentry{SPF-FF}

\addplot[
    no markers,
    dashed,
    color=orange,
    line width=0.9pt,
] table [x=episodes, y=ksp, col sep=comma] {data/erlang_750/k3/Pan-European/best_performing.csv};
\addlegendentry{KSP-FF $k=3$}

\end{axis}
\end{tikzpicture}

==> plots/erlang_750/Pan-European/k4.tex <==
% k4.tex

\begin{tikzpicture}
\begin{axis}[
    title={Pan-European Blocking Probability vs. Episodes},
    xlabel={Episodes},
    ylabel={Blocking Probability},
    grid,
    scaled y ticks=false,
    yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/fixed zerofill,
        /pgf/number format/precision=3,
    },
    xmax=100,
    xmin=-1,
    width=0.83\linewidth,
    height=0.73\linewidth,
    legend style={
        at={(0.99,0.8)},
        anchor=north east,
        legend cell align=left,
        font=\scriptsize,
    },
]

\addplot[
    no markers,
    solid,
    color=blue,
] table [x=episodes, y=q_learning, col sep=comma] {data/erlang_750/k4/Pan-European/best_performing.csv};
\addlegendentry{Q-Learning}

\addplot[
    no markers,
    solid,
    color=red,
    line width=0.9pt,
] table [x=episodes, y=epsilon_greedy_bandit, col sep=comma] {data/erlang_750/k4/Pan-European/best_performing.csv};
\addlegendentry{Epsilon-Greedy Bandit}

\addplot[
    no markers,
    solid,
    color=gray,
    line width=0.9pt,
] table [x=episodes, y=ucb_bandit, col sep=comma] {data/erlang_750/k4/Pan-European/best_performing.csv};
\addlegendentry{UCB Bandit}

\addplot[
    no markers,
    dashed,
    color=green,
    line width=0.9pt,
] table [x=episodes, y=spf, col sep=comma] {data/erlang_750/k4/Pan-European/best_performing.csv};
\addlegendentry{SPF-FF}

\addplot[
    no markers,
    dashed,
    color=orange,
    line width=0.9pt,
] table [x=episodes, y=ksp, col sep=comma] {data/erlang_750/k4/Pan-European/best_performing.csv};
\addlegendentry{KSP-FF $k=4$}

\end{axis}
\end{tikzpicture}

==> plots/erlang_750/Pan-European/k5.tex <==
% k5.tex

\begin{tikzpicture}
\begin{axis}[
    title={Pan-European Blocking Probability vs. Episodes},
    xlabel={Episodes},
    ylabel={Blocking Probability},
    grid,
    scaled y ticks=false,
    yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/fixed zerofill,
        /pgf/number format/precision=3,
    },
    xmax=100,
    xmin=-1,
    width=0.83\linewidth,
    height=0.73\linewidth,
    legend style={
        at={(0.99,0.8)},
        anchor=north east,
        legend cell align=left,
        font=\scriptsize,
    },
]

\addplot[
    no markers,
    solid,
    color=blue,
    line width=0.9pt,
] table [x=episodes, y=q_learning, col sep=comma] {data/erlang_750/k5/Pan-European/best_performing.csv};
\addlegendentry{Q-Learning}

\addplot[
    no markers,
    solid,
    color=red,
    line width=0.9pt,
] table [x=episodes, y=epsilon_greedy_bandit, col sep=comma] {data/erlang_750/k5/Pan-European/best_performing.csv};
\addlegendentry{Epsilon-Greedy Bandit}

\addplot[
    no markers,
    solid,
    color=gray,
    line width=0.9pt,
] table [x=episodes, y=ucb_bandit, col sep=comma] {data/erlang_750/k5/Pan-European/best_performing.csv};
\addlegendentry{UCB Bandit}

\addplot[
    no markers,
    dashed,
    color=green,
    line width=0.9pt,
] table [x=episodes, y=spf, col sep=comma] {data/erlang_750/k5/Pan-European/best_performing.csv};
\addlegendentry{SPF-FF}

\addplot[
    no markers,
    dashed,
    color=orange,
    line width=0.9pt,
] table [x=episodes, y=ksp, col sep=comma] {data/erlang_750/k5/Pan-European/best_performing.csv};
\addlegendentry{KSP-FF $k=5$}

\end{axis}
\end{tikzpicture}

==> plots/erlang_750/USNet/k3.tex <==
% k3.tex

\begin{tikzpicture}
\begin{axis}[
    title={USNet Blocking Probability vs. Episodes},
    xlabel={Episodes},
    ylabel={Blocking Probability},
    grid,
    scaled y ticks=false,
    yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/fixed zerofill,
        /pgf/number format/precision=3,
    },
    xmax=100,
    xmin=-1,
    width=0.83\linewidth,
    height=0.73\linewidth,
    legend style={
        at={(0.99,0.8)},
        anchor=north east,
        legend cell align=left,
        font=\scriptsize,
    },
]

\addplot[
    no markers,
    solid,
    color=blue,
    line width=0.9pt,
] table [x=episodes, y=q_learning, col sep=comma] {data/erlang_750/k3/USNet/best_performing.csv};
\addlegendentry{Q-Learning}

\addplot[
    no markers,
    solid,
    color=red,
    line width=0.9pt,
] table [x=episodes, y=epsilon_greedy_bandit, col sep=comma] {data/erlang_750/k3/USNet/best_performing.csv};
\addlegendentry{Epsilon-Greedy Bandit}

\addplot[
    no markers,
    solid,
    color=gray,
    line width=0.9pt,
] table [x=episodes, y=ucb_bandit, col sep=comma] {data/erlang_750/k3/USNet/best_performing.csv};
\addlegendentry{UCB Bandit}

\addplot[
    no markers,
    dashed,
    color=green,
    line width=0.9pt,
] table [x=episodes, y=spf, col sep=comma] {data/erlang_750/k3/USNet/best_performing.csv};
\addlegendentry{SPF-FF}

\addplot[
    no markers,
    dashed,
    color=orange,
    line width=0.9pt,
] table [x=episodes, y=ksp, col sep=comma] {data/erlang_750/k3/USNet/best_performing.csv};
\addlegendentry{KSP-FF $k=3$}

\end{axis}
\end{tikzpicture}

==> plots/erlang_750/USNet/k4.tex <==
% k4.tex

\begin{tikzpicture}
\begin{axis}[
    title={USNet Blocking Probability vs. Episodes},
    xlabel={Episodes},
    ylabel={Blocking Probability},
    grid,
    scaled y ticks=false,
    yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/fixed zerofill,
        /pgf/number format/precision=3,
    },
    xmax=100,
    xmin=-1,
    width=0.83\linewidth,
    height=0.73\linewidth,
    legend style={
        at={(0.99,0.8)},
        anchor=north east,
        legend cell align=left,
        font=\scriptsize,
    },
]

\addplot[
    no markers,
    solid,
    color=blue,
    line width=0.9pt,
] table [x=episodes, y=q_learning, col sep=comma] {data/erlang_750/k4/USNet/best_performing.csv};
\addlegendentry{Q-Learning}

\addplot[
    no markers,
    solid,
    color=red,
    line width=0.9pt,
] table [x=episodes, y=epsilon_greedy_bandit, col sep=comma] {data/erlang_750/k4/USNet/best_performing.csv};
\addlegendentry{Epsilon-Greedy Bandit}

\addplot[
    no markers,
    solid,
    color=gray,
    line width=0.9pt,
] table [x=episodes, y=ucb_bandit, col sep=comma] {data/erlang_750/k4/USNet/best_performing.csv};
\addlegendentry{UCB Bandit}

\addplot[
    no markers,
    dashed,
    color=green,
    line width=0.9pt,
] table [x=episodes, y=spf, col sep=comma] {data/erlang_750/k4/USNet/best_performing.csv};
\addlegendentry{SPF-FF}

\addplot[
    no markers,
    dashed,
    color=orange,
    line width=0.9pt,
] table [x=episodes, y=ksp, col sep=comma] {data/erlang_750/k4/USNet/best_performing.csv};
\addlegendentry{KSP-FF $k=4$}

\end{axis}
\end{tikzpicture}

==> plots/erlang_750/USNet/k5.tex <==
% k5.tex

\begin{tikzpicture}
\begin{axis}[
    title={USNet Blocking Probability vs. Episodes},
    xlabel={Episodes},
    ylabel={Blocking Probability},
    grid,
    scaled y ticks=false,
    yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/fixed zerofill,
        /pgf/number format/precision=3,
    },
    xmax=100,
    xmin=-1,
    width=0.83\linewidth,
    height=0.73\linewidth,
    legend style={
        at={(0.99,0.8)},
        anchor=north east,
        legend cell align=left,
        font=\scriptsize,
    },
]

\addplot[
    no markers,
    solid,
    color=blue,
    line width=0.9pt,
] table [x=episodes, y=q_learning, col sep=comma] {data/erlang_750/k5/USNet/best_performing.csv};
\addlegendentry{Q-Learning}

\addplot[
    no markers,
    solid,
    color=red,
    line width=0.9pt,
] table [x=episodes, y=epsilon_greedy_bandit, col sep=comma] {data/erlang_750/k5/USNet/best_performing.csv};
\addlegendentry{Epsilon-Greedy Bandit}

\addplot[
    no markers,
    solid,
    color=gray,
    line width=0.9pt,
] table [x=episodes, y=ucb_bandit, col sep=comma] {data/erlang_750/k5/USNet/best_performing.csv};
\addlegendentry{UCB Bandit}

\addplot[
    no markers,
    dashed,
    color=green,
    line width=0.9pt,
] table [x=episodes, y=spf, col sep=comma] {data/erlang_750/k5/USNet/best_performing.csv};
\addlegendentry{SPF-FF}

\addplot[
    no markers,
    dashed,
    color=orange,
    line width=0.9pt,
] table [x=episodes, y=ksp, col sep=comma] {data/erlang_750/k5/USNet/best_performing.csv};
\addlegendentry{KSP-FF $k=5$}

\end{axis}
\end{tikzpicture}
